Cost-Efficient Subjective Task Annotation and Modeling through Few-Shot Annotator Adaptation

In subjective NLP tasks, where a single ground truth does not exist, the inclusion of diverse annotators becomes crucial as their unique perspectives significantly influence the annotations. In realistic scenarios, the annotation budget often becomes the main determinant of the number of perspectives (i.e., annotators) included in the data and subsequent modeling. We introduce a novel framework for annotation collection and modeling in subjective tasks that aims to minimize the annotation budget while maximizing the predictive performance for each annotator. Our framework has a two-stage design: first, we rely on a small set of annotators to build a multitask model, and second, we augment the model for a new perspective by strategically annotating a few samples per annotator. To test our framework at scale, we introduce and release a unique dataset, Moral Foundations Subjective Corpus, of 2000 Reddit posts annotated by 24 annotators for moral sentiment. We demonstrate that our framework surpasses the previous SOTA in capturing the annotators' individual perspectives with as little as 25% of the original annotation budget on two datasets. Furthermore, our framework results in more equitable models, reducing the performance disparity among annotators.

==> sections/5.2old_results.tex <==
% In this section, first we present the results of our method compared the baseline 
% (\cref{sec:r1}).
% % Then we do an analysis of how different budgets affect performance on specifically high disagreement instances (\cref{sec:r_hig_dis}).
% We investigate how the disagreement of the initial annotators $A$ used for MTL training affect the final performance of the annotator adopted by a few shot  $A_{fs} $(\cref{sec:res_mtl})
% At last, we explore how the individual annotators' disagreement affects their FS performance (\cref{sec:fs_dis})
\subsection{Few Annotators are Enough} \label{sec: few_enough}
\input{tables/mtl_fs}
% One fundamental principle underlying past state-of-the-art methods for subjective tasks is that achieving performance gains is possible by jointly learning annotations from multiple annotators, as opposed to independently learning each annotator's perspectives. Here we investigate to what extent this principle is true. 
Previous state-of-the-art methods for subjective tasks achieve performance gains by jointly learning annotations from multiple annotators, as opposed to independently learning each annotator's perspectives \cite{davani2022dealing}. In this analysis, we further explore whether adding more annotators to the multitask model results in a better model for all annotators. To answer this question, we look at the multitask performance $F^{mtl}_1$ as the number of annotators in the multitask model, $|\mathcal{A}_{mtl}|$, grows. There is no statistically significant correlation between the number of annotators and $F_1^{mtl}$ ($r = -0.28, p > 0.05$). \autoref{fig:f1_n_mtl} shows that average $F^{mtl}_1$ for all annotators does not increase as the number of annotators increases. Note that this pattern is consistent in both datasets and as \autoref{fig:f1_n_mtl} shows, the $F^{mtl}_1$ scores are reliable with low standard deviations across models with different numbers of annotators. This observation motivates our first design choice; in the first stage of our framework, we can only rely on a small number of annotators to get a reliable multitask model.

\begin{figure}
  \centering
    % Subfigure 1
    \includegraphics[width=0.95\columnwidth]{figures/mlt_f1_vs_n_anns.png}
    \caption{Multitask models $F_1$ performance ($F_1^{mtl}$) as the number of annotators increase. Mean and standard deviation are reported across three repeated runs}
    \label{fig:f1_n_mtl}
    \vspace{-2mm}
\end{figure}





\subsection{Towards Better Performance with Less Annotation Budget} \label{sec:min_budget}
 A successful framework for modeling subjective tasks should, above all, demonstrate the ability to accurately predict labels from all of the annotators. Therefore, we assess the overall performance ($F^{\text{overall}}_1$) of our proposed framework in comparison to the baseline of multitask learning. 
 Recall the second component of our framework is to augment the multitask learning model of the first stage $\mathcal{F}_{mtl}$ to predict new annotators' labels using only a few samples. To isolate the impact of the few-shot learning model from the specific choice of samples, we sample the $k$ shots randomly. 
 
As shown in  \autoref{tab:overall-f1},  our framework outperforms the multitask baseline on both datasets when it comes to predicting labels of all annotators. 
Specifically, on MFSC, our approach outperforms multitask learning using 100\% of data with access to as little as 25\% of the original annotation budget. On Brexit, our framework matches the performance of multitask learning on 100\% budget with access to only 50\% of the original budget.
The findings demonstrate the success of our framework in achieving its dual objectives: enhancing performance across all annotators while reducing annotation budget requirements. Consequently, our framework facilitates increased diversity by incorporating additional annotator perspectives while adhering to a specific budget constraint.
We also conduct an ablation study by omitting the first MTL stage and employing random few-shot sampling for each annotator (Appendix \ref{sec:app-ablation}).
% Overall, these results demonstrate that our proposed framework succeeds in both of our objectives; improving performance on all annotators (i.e. performance maximization) while reducing the data requirements (i.e. annotation budget minimization).
 % Specifically, on Brexit, our approach outperforms multitask learning on full budget (100\%B) with access to only 66\% budget (k=128), and on \mf, our approach outperforms multitask learning with full data with as little as 25\% of the original annotation budget.
\input{tables/fs_sampling}
\subsection{Few-shot Sampling Strategies}
\label{sec:fs_sampling}
Recall that in the second stage of our framework, we only select a small subset of the input texts $\mathcal{S}(X) \subset X$ to be annotated by the new annotators (\autoref{fig:main}). Intuitively, we are relying on the first stage of our framework (i.e., multitask learning) to learn the commonalities between annotators. Hence, the goal of the selection function $\mathcal{S}(X)$ is to choose input texts that best capture individual annotators' differences. To study the impact of data selection strategies, we compare the fewshot performance ($F^{fs}_1$) of each strategy controlling for the number of shots $k$ (see \S \ref{sec:method} for definitions of $\mathcal{S(.)}$).

On Brexit dataset, the $\mathcal{S}_{bal}$ strategy, which selects a balanced sample for each annotator outperforms other approaches consistently with 50\% budget. With  66\% budget, $\mathcal{S}_{bal}$ strategy performs the best for all values of $k$. Notably, with this budget, the performance gap is closed by the $\mathcal{S}_{dis}$ for higher number of shots. Although the differences in performance are less pronounced for higher budget scenarios (i.e., the 83\%$B$), $\mathcal{S}_{bal}$ and $\mathcal{S}_{dis}$ still achieve better results especially when more shots are available. We acknowledge that the $\mathcal{S}_{bal}$ strategy relies on access to a balanced sample for each annotator which is often not readily available. However, this study showcases the potential of this approach and future work can explore methods that attempt to select instances that approximate a balanced sample per annotator.

On the \mf dataset, sampling strategies persistently outperform the multitask learning baseline in all scenarios. While different strategies seem to perform comparably, a crucial differentiating factor is the impact of various strategies on the stability of the results. Specifically, compared to $\mathcal{S}_{rand}$, all sampling functions result in more stable performances (i.e., lower standard deviation) across all budgets and values of $k$. 
% In the majority of scenarios, $\mathcal{S}_{bal}$ achieves most stable results among all variants. 

Overall, our results on two datasets show that the fewshot stage of our framework, results in models that consistently outperform the multitask learning baseline. Our experiments clearly demonstrate the importance of sample selection strategies both in terms of performance improvement and stability. Furthermore, our results on both datasets motivate the exploration of sampling strategies that can approximate a balanced sample per annotator.

\subsection{Reduced Performance Disparities across Annotators} \label{sec:dispar}
% Fairness in classification is important. One way that models may cause harm is through performance disparities. timnit cite. 
   % In comparison to the standard practice of machine learning in modeling the majority label, our goal is to incorporate and capture diverse perspectives from all annotators.
  
Ensuring a comprehensive representation of annotators' viewpoints is crucial in modeling subjective tasks. To achieve this goal, a critical criterion is to create models that not only improve the aggregated performance but also demonstrate fair and equitable performance across all annotators. For example, if the $F_1$ scores of one model for two annotators are 0.6 and 0.8, respectively, while the second model scores 0.7 for both annotators, the latter is considered a better model. Although the average performance is the same for both models, the first model has a disparate negative impact on the first annotator.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{figures/brexit_dispar.png}
    \caption{Comparison of Annotator level F1 scores ($F_1^{a_i}$) on the Brexit dataset between MTL model and our framework, leveraging the $\mathcal{S}_{bal}$ sampling method for all budgets and shots}
    \label{fig:brexit-fairness} 
    \vspace{-5mm}
\end{figure}
This is important because performance disparities among social groups (in our case annotators) can lead to biased models, limiting the system's ability to accurately reflect diverse perspectives and potentially perpetuating inequalities in the outputs of subjective tasks \citep{buolamwini2018gender}.
Merely relying on aggregated performance measures, like the average across all annotators, falls short of providing a complete understanding of how well the model is capturing annotators' varying perspectives. For example, it is not clear whether the average performance is improving because an approach improves on capturing only a subset of annotators or for everyone. 
Hence, we look into the standard deviation of performance across all annotators $d = \sqrt{\frac{1}{N-1} \sum_{i=1}^N (F^{a_i}_1 - \overline{F^{overall}_1})^2}$. Lower standard deviations are indicative of more equitable models.

As shown in \autoref{tab:variance}, regardless of the sampling strategy, our approach results in lower performance variances compared to the MTL baseline on lower budgets (50\% and 66\%). Comparing the different sampling strategies on Brexit dataset, we observe that $S_{bal}$ achieves the most equitable models across all values of $k$. On MFSC, using a balanced sampling strategy consistently reduces the disparities among annotators compared to the MTL baseline for all budgets. \autoref{fig:brexit-fairness} visualizes the performance of our framework in comparison to the multitask learning baseline for each annotator. Notably, our framework improves the performance for the annotators in the non-Western control group (i.e., the first three annotators)  while maintaining the performance of the rest of the annotators.

Overall, these results suggest that our proposed framework not only improves the overall performance of all annotators but also yields models that are more fair and equitable. Interestingly, we observe similar patterns in fairness and overall performance improvements. In other words, the configurations with the best overall performance (see section \ref{sec:fs_sampling})  are also the ones that have the least performance disparities among all annotators.

 \input{tables/annotator_variance}

==> sections/old_results/5.0.results_performance.tex <==
\subsection{New Annotator Adaptation} \label{sec:r1}

% The aggregated results are shown in Table \ref{tab:results}. The annotator level results are presented in Figure \ref{fig:overall}. 

The aggregated results are shown in Table \ref{tab:main_res}. The first row of the table indicates the baseline results. As it is apparent from the table, our method overall outperfomrs the baseline with all three methods of sampling. Specifically, for Brexit dataset the f1 of the baseline with full budget is 0.43, meanwhile with $\mathcal{S}_{bal}$ and only 50\% outperforms with f1 score of 0.5 .$\mathcal{S}_{dis}$ is the second best performing with performance boost of 8\% in f1 score, with 83\% of the budget and k=64.

For MFRC dataset the best performing model is with $\mathcal{S}_mv$ with 25\% of the budget, with 3\% increase in f1 compared to baseline with full budget.

The annotator level results are presented in Figure \ref{fig:overall}. 

% \setlength{\tabcolsep}{5pt}
% \begin{table}[h!]
%     \centering
%     \caption{Aggregated F1 results on BREXIT dataset for different budgets of annotation, selection method: balanced mv with weighted sampler}
%     \label{tab:mfrc}
%     \begin{tabular}{cc|cccc}
%         \toprule
%       &  & 0.5 & 0.66 & 0.83 & 1.0 \\ \hline
%         & MTL &  0.459 & 0.467 & 0.429 & 0.432 \\ \hline
%         \multirow{4}{*}{\rotatebox[origin=l]{90}{Few shot}} 
%         & 8& 0.420 & 0.420 & 0.504 & \cellcolor{lightgray} \\
%         & 16 & 0.394 & 0.436 & 0.434 & \cellcolor{lightgray} \\
%         & 32 & 0.424 & 0.437 & 0.460 & \cellcolor{lightgray} \\
%         & 64 & 0.425 & 0.437 & 0.487 & \cellcolor{lightgray} \\
%         \bottomrule
%     \end{tabular}
% \end{table}


% \begin{table}
% \caption{Aggregate F1 results on  mfrc dataset, selection method : balanced mv}
% \label{tab:mfrc}
% \begin{tabular}{lllll}
% \toprule
% budget & 0.25 & 0.5 & 0.75 & 1.0 \\
% k-shot &  &  &  &  \\
% \midrule
% 0 & 0.763_{(0.016)} & 0.773_{(0.011)} & 0.772_{(0.015)} & 0.776_{(0.004)} \\
% 16 & 0.799_{(0.003)} & 0.794_{(0.004)} & 0.786_{(0.015)} & NaN \\
% 32 & 0.801_{(0.003)} & 0.795_{(0.003)} & 0.787_{(0.017)} & NaN \\
% 64 & 0.802_{(0.004)} & 0.797_{(0.002)} & 0.79_{(0.018)} & NaN \\
% 128 & 0.805_{(0.004)} & 0.798_{(0.003)} & 0.79_{(0.019)} & NaN \\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}
% \caption{Aggregate F1 results on  brexit dataset, selection method : balanced mv}
% \label{tab:brexit}
% \begin{tabular}{lllll}
% \toprule
% budget & 0.5 & 0.66 & 0.83 & 1.0 \\
% k-shot &  &  &  &  \\
% \midrule
% 0 & 0.417_{(0.049)} & 0.449_{(0.027)} & 0.418_{(0.018)} & 0.431_{(0.014)} \\
% 16 & 0.409_{(0.018)} & 0.416_{(0.026)} & 0.442_{(0.055)} & NaN \\
% 32 & 0.404_{(0.029)} & 0.426_{(0.029)} & 0.461_{(0.024)} & NaN \\
% 64 & 0.409_{(0.017)} & 0.41_{(0.05)} & 0.467_{(0.011)} & NaN \\
% 128 & 0.425_{(0.028)} & 0.428_{(0.035)} & 0.46_{(0.025)} & NaN \\
% \bottomrule
% \end{tabular}
% \end{table}



% \setlength{\tabcolsep}{5pt}
% \begin{table}[h!]
%     \centering
%     \caption{Aggregated F1 results on MFRC dataset for different budgets of annotation, selection method: balanced mv}
%     \label{tab:mfrc}
%     \begin{tabular}{cc|cccc}
%         \toprule
%       &  & 0.25 & 0.5 & 0.75 & 1.0 \\ \hline
%         & MTL & 0.769 & 0.782 & 0.784 & 0.775 \\ \hline
%         \multirow{4}{*}{\rotatebox[origin=l]{90}{Few shot}} 
%         & 8 & 0.802 & 0.799 & 0.804 & \cellcolor{lightgray} \\
%         & 16 & 0.804 & 0.798 & 0.806 & \cellcolor{lightgray} \\
%         & 32 & 0.806 & 0.799 & 0.811 & \cellcolor{lightgray} \\
%         & 64 & 0.810 & 0.801 & 0.812 & \cellcolor{lightgray} \\
%         \bottomrule
%     \end{tabular}
% \end{table}












==> sections/old_results/5.1.result_high_dis.tex <==

\subsection{Budget and High Disagreement Intances} \label{sec:r_hig_dis}

\begin{figure*}[t!]
  \centering
    % Subfigure 1
     \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/brexit_aggr_high_dis.png}
    \caption{BREXIT}
    \label{fig:brexit_plot}
    \end{subfigure}
    % Subfigure 2
   \hfill
       \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth]{figures/mfrc_aggr_high_dis.png}
        \caption{MFRC}
        \label{fig:mfrc-plot}
    \end{subfigure}

    \caption{Aggreget performance on high disagreement samples across different budgets}
\end{figure*}




% \setlength{\tabcolsep}{5pt}
% \begin{table}[h!]
% \caption{Aggregate F1 results on  brexit \textbf{high disagreement} dataset, selection method : balanced mv}
% \label{tab:brexit}
% \begin{tabular}{cc|cccc}
% \toprule
% &  & 0.5 & 0.66 & 0.83 & 1.0 \\ \hline
% & MTL & 0.646 & 0.602 & 0.490 & 0.672 \\ \hline
% \multirow{4}{*}{\rotatebox[origin=l]{90}{Few shot}} 
% & 16 & 0.477 & 0.414 & 0.576 &  \cellcolor{lightgray}  \\
% & 32 & 0.407 & 0.429 & 0.423 & \cellcolor{lightgray}  \\
% & 64 & 0.462 & 0.452 & 0.437 &  \cellcolor{lightgray}  \\
% & 128 & 0.447 & 0.454 & 0.523 &  \cellcolor{lightgray}  \\
% \bottomrule
% \end{tabular}
% \end{table}


% \setlength{\tabcolsep}{5pt}
% \begin{table}[h!]
%     \centering
%     \caption{Aggregated F1 results on MFRC \textbf{high disagreement test set} dataset for different budgets of annotation, selection method: balanced mv}
%     \label{tab:mfrc}
%     \begin{tabular}{cc|cccc}
%         \toprule
%       &  & 0.25 & 0.5 & 0.75 & 1.0 \\ \hline
%         & MTL & 0.652 & 0.655 & 0.650 & 0.626 \\ \hline
%         \multirow{4}{*}{\rotatebox[origin=l]{90}{Few shot}} 
%         & 8 & 0.649 & 0.639 & 0.648 & \cellcolor{lightgray} \\
%         & 16 & 0.657 & 0.644 & 0.646 &  \cellcolor{lightgray} \\
%         & 32 & 0.674 & 0.653 & 0.670 & \cellcolor{lightgray} \\
%         & 64 & 0.674 & 0.653 & 0.670 & \cellcolor{lightgray} \\
%         \bottomrule
%     \end{tabular}
% \end{table}


==> sections/old_results/5.2.result_mtl-stable.tex <==
\subsection{MTL disagreement and few shot performance} \label{sec:res_mtl}
\begin{figure*}[t!]
  \centering
    % Subfigure 1
     \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\columnwidth, ]{figures/analysis_2_scatter_brexit_dis_f1.png}
    \caption{BREXIT}
    \end{subfigure}
    % Subfigure 2
   \hfill
       \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\columnwidth, ]{figures/analysos_2_scatter_mfrc_dis_f1.png}
        \caption{MFRC}
    \end{subfigure}
    \caption{ Disagreement of $A$ and F1 of $A_{fs}$}
    \label{fig:mtl-dis-f1}
\end{figure*}

\begin{figure*}[t!]
  \centering
    % Subfigure 1
     \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\columnwidth, height=2.1in]{figures/analysis_3_brexit_fs_dis_f1.png}
    \caption{BREXIT}
    \end{subfigure}
    % Subfigure 2
   \hfill
       \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\columnwidth, height=2.1in]{figures/analysis_3_mfrc_fs_dis_f1.png}
        \caption{MFRC}
    \end{subfigure}
    \caption{ Disagreement of $A_{fs}$ with $A$ and F1 of $A_{fs}$}
    \label{fig:fs-dis-f1}
\end{figure*}
% In our experiments, we adopt a new task as a few-shot on top of different combinations of MTL-trained annotators. We do this to ensure that a new annotator is not only working on top of a specific set of annotators because we don't have that in real-world problem settings. The initial annotators that we run the mtl on can have varying levels of disagreement with each other; for example, they might have perfect agreement, or on the other side of the spectrum, they might all disagree on all the instances. 
The objective of this analysis is to investigate how the degree of disagreement within the set $\mathcal{A}_{mt}$ influences the performance of the newly adopted annotators, denoted as $A_{fs}$. This exploration is crucial for guiding the selection process of the initial annotator set $\mathcal{A}_{mt}$.

% % In this analysis, we are analyzing how different levels of disagreement of $\mathcal{A}_{mtl$ affect the performance of newly adopted annotators $A_{fs}$.

% This is important because if there is a relationship, then it can guide us for the selection of the set $A$, and if there is not a relationship, then there is less restriction on choosing the set $A$.

To test this relationship we run a mixed effects model to predict the performance of $a \in \mathcal{A}_{fs}$ by the independent variable Fleiss kappa agreement measure of $\mathcal{A}_{mt}$, while controlling for $k$ and  buget, and including random effects for $\mathcal{A}_{mt}$ and $\mathbf{A}_{fs}$. 

% There was no significant effect for fless agreement on the performance 
These results suggest that variations in Fleiss agreement within $\mathcal{A}_mt$ do not have a statistically significant impact on the performance of the $A_{fs}$ for either of the datasets (MFRC : $\beta = 0.013 , SE = 0.024, p =  0.595$ , Brexit : $\beta = 0.097 , SE = 0.11, p =  0.393$ ). The detailed plots can be found in Figure \ref{fig:mtl-dis-f1}.


==> sections/old_results/5.3.result_fs_dis.tex <==
\subsection{New Annotator Adaptation with Different Levels of Disagreement} \label{sec:fs_dis}


% As it is apparent in annotator level results in figure \ref{fig:mfrc-plot} and \ref{fig:brexit_plot}, For some annotators the performance gap is larger than for others. For example, annotators 18 to 23  in figure \ref{fig:mfrc-plot} have over 10\% performance gain when learned as fewshot task, rather than as a task in an MTL setting with a full budget. 
% % For this method to be generalizable and actually practical for new annotator adaptation, it is important to study whether the disagreement of some annotators is not the main driver of their few-shot performance.

The annotator-level results depicted in Figure \ref{fig:mfrc-plot} and \ref{fig:brexit_plot} reveal notable variations in the performance gap among annotators. Specifically, in Figure \ref{fig:mfrc-plot}, annotators 18 to 23 demonstrate a performance gain exceeding 10\% when learning in a few-shot setting as opposed to being part of an MTL task with a full budget.

In this analysis we test weather the disagreement between $\mathcal{A}_{fs}$ and $\mathcal{A}_{mt}$ affects the performance of $\mathcal{A}_{fs}$.
For this we also ran a mixed effect model, predicting the f1 of  $\mathcal{A}_{fs}$, with the disagreement , and controlling for $k$ and budget.
For Brexit dataset, our findings suggest no substantial impact ($\beta = 0.077 , SE = 0.46, p = 0.867$). However, for MFRC, the results indicate a significant effect (MFRC: $\beta = 0.059 , SE = 0.017, p < 0.001$), signifying that a one-unit increase in agreement is correlated with a 0.059 increase in F1.
% To ensure the generalizability and practicality of this method for new annotator adaptation, it becomes important to investigate whether a particular characteristic of certain annotators is the primary driver behind their enhanced few-shot performance.
The annotator level plots are shown in Figure \ref{fig:fs-dis-f1}. 



==> sections/t_test.tex <==
\textbf{MFSC and Brexit}
In this dataset of our experiments, all instances are annotated by all annotators. However, this is not the case in so many datasets. So, in order to test the impact of the imbalanced number of annotations on the performance of our framework we conduct a statistical analysis by dividing annotators into two groups: one with fewer annotations ($k=32$) and the other with more annotations ($k=128$). We used a t-test to compare the $F_1$ scores between these groups and reported Cohen’s d effect size for precise measurement. The results in \autoref{tab:imbalance_impact} show significantly higher $F_1$ scores for the group with more annotation for the Brexit dataset while indicating no significant difference for the MFSC dataset.
With that said, it's essential to emphasize that our framework design leads to enhanced results for annotators with only a few-shot annotation, compared to the baseline approach with a larger number of annotations. Essentially, our framework effectively tackles the impact of data imbalance on performance.

\begin{table}[h!]
\centering
\begin{tabular}{@{}lccc@{}} \toprule
Dataset & {T-statistic} & {P-value} & {Cohen’s d} \\
\midrule
Brexit & -3.46 & 0.002 & 0.77 \\
MFSC & -1.59 & 0.114 & 0.15 \\
\bottomrule
\end{tabular}
\caption{Comparison of T-statistic, P-value, and Cohen’s d for Brexit and MFSC datasets.}
\label{tab:imbalance_impact}
\end{table}

==> tables/annotator_variance.tex <==




% \begin{table}[h!]
% \small
% \begin{tabular}{ll|lll|lll}
% \toprule  & & \multicolumn{3}{c|}{Brexit} & \multicolumn{3}{c}{Multipers-mfrc} \\
% & $\%B_f$ & $50\%$ &    $66\%$ & $83\%$ & $25\%$ & $50\%$ & $75\%$ \\
% \midrule
% \multicolumn{2}{c|}{MTL} & .168 & .139 & .131 &  .128 & .136 & .127 \\ \hline
% \multirow[c]{4}{*}{$\mathcal{S}_{bal}$} 
%  & $k=16$ & .119 & .127 & .132 & .119 & .124 & .124 \\
%  &  $k=32$ & .113 & .125 & .133 & .120 & .125 & .124 \\
%  &  $k=64$ & .109 & .119 & .127 & .119 & .124 & .123 \\
%  & $k=128$ & \textbf{.093} & \textbf{.108} & \textbf{.117} &.\textbf{117} & \textbf{.122} & \textbf{.121} \\
% \cline{1-8}
% \multirow[c]{4}{*}{$\mathcal{S}_{dis}$} 
%  &  $k=16$ & .141 & .134 & .127 & .129 & .130 & \textbf{.126} \\
%  &  $k=32$ & .145 & .138 & .131 &  .131 & .130 & .126 \\
%  & $k=64$ & .137 & .126 & \textbf{.123} & .131 & .130 & .126 \\
%  & $k=128$  & \textbf{.111} & \textbf{.120} & .124 &  .130 & \textbf{.129} & .127 \\
% \cline{1-8}
% \multirow[c]{4}{*}{$\mathcal{S}_{mv}$} 
%  &  $k=16$ & .138 & \textbf{.137} & .131 &  .131 & .130 & .127 \\
%  &  $k=32$ & .140 & .137 & .129 &  .130 & .130 & .127 \\
%  & $k=64$ & .145 & .146 & \textbf{.126} &  .130 & .129 & .127 \\
%  & $k=128$ & \textbf{.137} & .142 & .132  & \textbf{.126} & \textbf{.128} & .127 \\
% \cline{1-8}
% \multirow[c]{4}{*}{$\mathcal{S}_{rand}$} 
%  &  $k=16$ & .137 & .139 & .135 &  \textbf{.137} & .135 & .130 \\
%  &  $k=32$ & .139 & .135 & .138 &  .136 & .134 & .129 \\
%  & $k=64$ & \textbf{.131} & .128 & .132 &  .136 & .135 & .129 \\
%  & $k=128$  & .131 & \textbf{.127} & .136  & .134 & .133 & .128 \\
% \cline{1-8}
% \bottomrule
% \end{tabular}
% \caption{ $d \downarrow$ performance across annotators, for full budget $d=.13$ for both datasets}
% \label{tab:variance}
% \end{table}

\renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{4pt}
\begin{table}\small
\begin{tabular}{ll|lll|lll}
% \toprule
\Xhline{3\arrayrulewidth}
 \multicolumn{2}{c|}{\multirow{2}{*}{$metric = d \downarrow$}} & \multicolumn{3}{c|}{Brexit} & \multicolumn{3}{c}{\mf} \\  
\multicolumn{2}{c|}{} & $50\%$ &    $66\%$ & $83\%$ & $25\%$ & $50\%$ & $75\%$ \\ \Xhline{2\arrayrulewidth}
% \midrule
 \multicolumn{2}{c|}{MTL} & .168 & .139 & .131 &  .128 & .136 & .127 \\ \hline
\multirow[c]{4}{*}{$k=16$} & $\mathcal{S}_{bal}$ & .119 & .127 & .132 & .119 & .124 & .124 \\
 & $\mathcal{S}_{dis}$ & .141 & .134 & .127 & .129 & .130 & .126 \\
 & $\mathcal{S}_{mv}$ & .138 & .137 & .131 & .131 & .130 & .127 \\  
 & $\mathcal{S}_{rand}$ & .137 & .139 & .135 & .137 & .135 & .130 \\  \hline\hline
% \cline{1-8} 
\multirow[c]{4}{*}{$k=32$} & $\mathcal{S}_{bal}$ & .113 & .125 & .133 & .120 & .125 & .124 \\
 & $\mathcal{S}_{dis}$ & .145 & .138 & .131 & .131 & .130 & .126 \\
 & $\mathcal{S}_{mv}$ & .140 & .137 & .129 & .130 & .130 & .127 \\
 & $\mathcal{S}_{rand}$ & .139 & .135 & .138 & .136 & .134 & .129 \\ \hline\hline
% \cline{1-8} 
\multirow[c]{4}{*}{$k=64$} & $\mathcal{S}_{bal}$ & .109 & .119 & .127 & .119 & .124 & .123 \\
 & $\mathcal{S}_{dis}$ & .137 & .126 & .123 & .131 & .130 & .126 \\
 & $\mathcal{S}_{mv}$ & .145 & .146 & .126 & .130 & .129 & .127 \\
 & $\mathcal{S}_{rand}$ & .131 & .128 & .132 & .136 & .135 & .129 \\ \hline\hline
% \cline{1-8}
\multirow[c]{4}{*}{$k=128$} & $\mathcal{S}_{bal}$ & \textbf{.093} & \textbf{.108} & \textbf{.117} & \textbf{.117} & \textbf{.122} & \textbf{.121} \\
 & $\mathcal{S}_{dis}$ & .111 & .120 & .124 & .130 & .129 & .127 \\
 & $\mathcal{S}_{mv}$ & .137 & .142 & .132 & .126 & .128 & .127 \\
 & $\mathcal{S}_{rand}$ & .131 & .127 & .136 & .134 & .133 & .128 \\ \hline
\cline{1-8}
% \bottomrule
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{ $d \downarrow$ measure across annotators, for full budget $d=.13$ for both datasets; $\mathcal{S}_{bal}$, $\mathcal{S}_{dis}$, $\mathcal{S}_{mv}$, and $\mathcal{S}_{rand}$ refer to the sampling functions used in the second stage of our framework (\S \ref{sec:method})}
\label{tab:variance}
\vspace{-5mm}
\end{table}







% \begin{table*}[h!]\small
% \caption{Variance of performance across annotators}
% \label{tab:variance}
% \begin{tabular}{ll|lll|lll}
% \toprule & & \multicolumn{3}{c|}{Brexit} & \multicolumn{3}{c}{mfrc} \\
%  &  & .5_x & .66 & .83 & .25 & .5_y & .75 \\
% sampling & k_shot &  &  &  &  &  &  \\
% \midrule
% \multirow[t]{4}{*}{$\mathcal{S}_{bal}$} & $k=128$ & .471\textsubscript{\hl{(.093)}} & .474\textsubscript{\hl{(.108)}} & .468\textsubscript{\hl{(.117)}} & .781\textsubscript{\hl{(.117)}} & .781\textsubscript{\hl{(.122)}} & .78\textsubscript{\hl{(.121)}} \\
%  & $k=16$ & .443\textsubscript{(.119)} & .454\textsubscript{(.127)} & .456\textsubscript{(.132)} & .777\textsubscript{(.119)} & .78\textsubscript{(.124)} & .779\textsubscript{(.124)} \\
%  & $k=32$ & .449\textsubscript{(.113)} & .458\textsubscript{(.125)} & .458\textsubscript{(.133)} & .779\textsubscript{(.12)} & .78\textsubscript{(.125)} & .779\textsubscript{(.124)} \\
%  & $k=64$ & .453\textsubscript{(.109)} & .458\textsubscript{(.119)} & .459\textsubscript{(.127)} & .779\textsubscript{(.119)} & .781\textsubscript{(.124)} & .78\textsubscript{(.123)} \\
% \cline{1-8}
% \multirow[t]{4}{*}{$\mathcal{S}_{dis}$} & $k=128$ & .45\textsubscript{(.111)} & .461\textsubscript{(.12)} & .466\textsubscript{(.124)} & .791\textsubscript{(.13)} & .789\textsubscript{(.129)} & .783\textsubscript{(.127)} \\
%  & $k=16$ & .421\textsubscript{(.141)} & .439\textsubscript{(.134)} & .457\textsubscript{(.127)} & .787\textsubscript{(.129)} & .787\textsubscript{(.13)} & .782\textsubscript{(.126)} \\
%  & $k=32$ & .423\textsubscript{(.145)} & .44\textsubscript{(.138)} & .457\textsubscript{(.131)} & .789\textsubscript{(.131)} & .788\textsubscript{(.13)} & .783\textsubscript{(.126)} \\
%  & $k=64$ & .436\textsubscript{(.137)} & .455\textsubscript{(.126)} & .468\textsubscript{(.123)} & .79\textsubscript{(.131)} & .789\textsubscript{(.13)} & .783\textsubscript{(.126)} \\
% \cline{1-8}
% \multirow[t]{4}{*}{$\mathcal{S}_{mv}$} & $k=128$ & .434\textsubscript{(.137)} & .445\textsubscript{(.142)} & .458\textsubscript{(.132)} & .793\textsubscript{(.126)} & .788\textsubscript{(.128)} & .782\textsubscript{(.127)} \\
%  & $k=16$ & .426\textsubscript{(.138)} & .441\textsubscript{(.137)} & .455\textsubscript{(.131)} & .789\textsubscript{(.131)} & .786\textsubscript{(.13)} & .782\textsubscript{(.127)} \\
%  & $k=32$ & .424\textsubscript{(.14)} & .444\textsubscript{(.137)} & .458\textsubscript{(.129)} & .79\textsubscript{(.13)} & .787\textsubscript{(.13)} & .782\textsubscript{(.127)} \\
%  & $k=64$ & .427\textsubscript{(.145)} & .439\textsubscript{(.146)} & .459\textsubscript{(.126)} & .791\textsubscript{(.13)} & .788\textsubscript{(.129)} & .782\textsubscript{(.127)} \\
% \cline{1-8}
% \multirow[t]{4}{*}{$\mathcal{S}_{rand}$} & $k=128$ & .439\textsubscript{(.131)} & .457\textsubscript{(.127)} & .455\textsubscript{(.136)} & .789\textsubscript{(.134)} & .784\textsubscript{(.133)} & .781\textsubscript{(.128)} \\
%  & $k=16$ & .422\textsubscript{(.137)} & .44\textsubscript{(.139)} & .455\textsubscript{(.135)} & .786\textsubscript{(.137)} & .783\textsubscript{(.135)} & .78\textsubscript{(.13)} \\
%  & $k=32$ & .428\textsubscript{(.139)} & .447\textsubscript{(.135)} & .452\textsubscript{(.138)} & .786\textsubscript{(.136)} & .783\textsubscript{(.134)} & .78\textsubscript{(.129)} \\
%  & $k=64$ & .433\textsubscript{(.131)} & .451\textsubscript{(.128)} & .456\textsubscript{(.132)} & .787\textsubscript{(.136)} & .783\textsubscript{(.135)} & .78\textsubscript{(.129)} \\
% \cline{1-8}
% \bottomrule
% \end{tabular}
% \end{table*}



% \begin{table*}[h!]
% \small
% \caption{Variance across annotators baseline }
% \label{tab:variance_baseline}
% \begin{tabular}{lllllllll}
% \toprule
% budget & .5 & .66 & .83 & 1.0 & .25 & .5 & .75 & 1.0 \\
% \midrule
% f1 & .417(.168) & .449(.139) & .418(.131) & .431(.13) & .763(.128) & .773(.136) & .772(.127) & .776(.13) \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> tables/care_fs.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{1pt}
\begin{table}[h!]\small
\begin{tabular}{cc|cccc}
\toprule   \multicolumn{2}{c|}{$metric = F_1^{fs} \uparrow$}  &  \multicolumn{4}{c}{MFSC(Care)} \\
 \multicolumn{2}{c|}{$\%B$} & $25\%$ & $50\%$  & $75\%$  &  $100\%$ \\
\midrule
\multicolumn{2}{c|}{MTL} &  0.474 & 0.476 & 0.49 & 0.469 \\ \hline

 \multicolumn{2}{c|}{$\%B$ $(\frac{\lvert \mathcal{A}_{mtl} \rvert}{\lvert \mathcal{A} \rvert})$} & $25\%$ $(\frac{6}{24})$ &  $50\%$ $(\frac{12}{24})$ & $75\%$ $(\frac{18}{24})$ &  $100\%$  $(\frac{24}{24})$\\ \hline
\multirow[c]{4}{*}{16} & $\mathcal{S}_{bal}$ & 0.450 & 0.446 & 0.478  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{dis}$ & 0.448 & 0.436 & 0.477 & \cellcolor{lightgray}  \\
 & $\mathcal{S}_{mv}$ & 0.470 & 0.449 & \textbf{0.496}  & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.459 & 0.439 & 0.467   & \cellcolor{lightgray}\\
\cline{1-6}
\multirow[c]{4}{*}{32} & $\mathcal{S}_{bal}$ & 0.457 & 0.457 & 0.487  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{dis}$ & 0.452 & 0.429 & 0.469  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{mv}$ & 0.468 & 0.453 & 0.491  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{rand}$ & 0.461 & 0.439 & 0.475  & \cellcolor{lightgray} \\
\cline{1-6}
\multirow[c]{4}{*}{64} & $\mathcal{S}_{bal}$ & 0.461 & 0.453 & 0.482  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{dis}$ & 0.457 & 0.444 & 0.449  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{mv}$ & 0.473 & 0.463 & 0.486  & \cellcolor{lightgray}\\
 & $\mathcal{S}_{rand}$ & 0.464 & 0.456 & 0.497  & \cellcolor{lightgray}\\
\cline{1-6}
\multirow[c]{4}{*}{128} & $\mathcal{S}_{bal}$ & 0.465 & 0.457 & 0.490  & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.467 & 0.452 & 0.462  & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.471 & 0.466 & 0.489  & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & \textbf{0.479 }& 0.464 & 0.485  & \cellcolor{lightgray}\\
\cline{1-6}
\bottomrule
\end{tabular}
\caption{Aggregated few shot $F_1$ results on MFRC, Care moral concern dataset for different $\%B_f$s of annotation.}
\label{tab:main_res}
\end{table}



==> tables/fs_sampling.tex <==
% \begin{table*}[h!]\small
% \begin{tabular}{cl|llll|llll}
% \toprule  & & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{mfrc} \\
%  & $\%B_f$ & $50\%$ & $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\

% \midrule
% \multicolumn{2}{c|}{MTL} & 0.417\textsubscript{(0.049)} & 0.449\textsubscript{(0.027)} & 0.418\textsubscript{(0.018)} & 0.431\textsubscript{(0.014)} & 0.763\textsubscript{(0.016)} & 0.773\textsubscript{(0.011)} & 0.772\textsubscript{(0.015)} & 0.776\textsubscript{(0.004)} \\
% \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{bal}$} & $k=16$ & 0.442\textsubscript{(0.003)} & 0.457\textsubscript{(0.016)} & 0.458\textsubscript{(0.044)} & \cellcolor{lightgray} & 0.785\textsubscript{(0.006)} & 0.781\textsubscript{(0.004)} & 0.778\textsubscript{(0.01)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.454\textsubscript{(0.013)} & 0.469\textsubscript{(0.004)} & 0.461\textsubscript{(0.026)} & \cellcolor{lightgray} & 0.787\textsubscript{(0.006)} & 0.782\textsubscript{(0.003)} & 0.779\textsubscript{(0.012)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.462\textsubscript{(0.01)} & 0.47\textsubscript{(0.018)} & 0.467\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.788\textsubscript{(0.005)} & 0.784\textsubscript{(0.001)} & 0.782\textsubscript{(0.011)} & \cellcolor{lightgray} \\
%  & $k=128$ & 0.498\textsubscript{(0.009)} & 0.517\textsubscript{(0.025)} & 0.524\textsubscript{(0.021)} & \cellcolor{lightgray} & 0.79\textsubscript{(0.005)} & 0.785\textsubscript{(0.001)} & 0.785\textsubscript{(0.01)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{dis}$} & $k=16$ & 0.399\textsubscript{(0.013)} & 0.412\textsubscript{(0.006)} & 0.457\textsubscript{(0.036)} & \cellcolor{lightgray} & 0.793\textsubscript{(0.01)} & 0.795\textsubscript{(0.004)} & 0.785\textsubscript{(0.01)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.402\textsubscript{(0.008)} & 0.413\textsubscript{(0.02)} & 0.455\textsubscript{(0.03)} & \cellcolor{lightgray} & 0.796\textsubscript{(0.01)} & 0.797\textsubscript{(0.004)} & 0.787\textsubscript{(0.011)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.429\textsubscript{(0.018)} & 0.458\textsubscript{(0.018)} & 0.518\textsubscript{(0.017)} & \cellcolor{lightgray} & 0.797\textsubscript{(0.011)} & 0.799\textsubscript{(0.005)} & 0.788\textsubscript{(0.012)} & \cellcolor{lightgray} \\
%  & $k=128$ & 0.456\textsubscript{(0.011)} & 0.476\textsubscript{(0.026)} & 0.511\textsubscript{(0.023)} & \cellcolor{lightgray} & 0.798\textsubscript{(0.009)} & 0.799\textsubscript{(0.003)} & 0.786\textsubscript{(0.012)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{mv}$} & $k=16$ & 0.409\textsubscript{(0.018)} & 0.416\textsubscript{(0.026)} & 0.442\textsubscript{(0.055)} & \cellcolor{lightgray} & 0.799\textsubscript{(0.003)} & 0.794\textsubscript{(0.004)} & 0.786\textsubscript{(0.015)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.404\textsubscript{(0.029)} & 0.426\textsubscript{(0.029)} & 0.461\textsubscript{(0.024)} & \cellcolor{lightgray} & 0.801\textsubscript{(0.003)} & 0.795\textsubscript{(0.003)} & 0.787\textsubscript{(0.017)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.409\textsubscript{(0.017)} & 0.41\textsubscript{(0.05)} & 0.467\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.802\textsubscript{(0.004)} & 0.797\textsubscript{(0.002)} & 0.79\textsubscript{(0.018)} & \cellcolor{lightgray} \\
%  & $k=128$ & 0.425\textsubscript{(0.028)} & 0.428\textsubscript{(0.035)} & 0.46\textsubscript{(0.025)} & \cellcolor{lightgray} & 0.805\textsubscript{(0.004)} & 0.798\textsubscript{(0.003)} & 0.79\textsubscript{(0.019)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \bottomrule
% \end{tabular}
% \caption{Aggregated F1 results on BREXIT  and MFRC dataset for different $\%B_f$s of annotation, mean and std over 3  runs}
% \label{tab:main_res}
% \end{table*}
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{5pt}

% \begin{table*}[h!]\small
% \begin{tabular}{cl|llll|llll}
% \toprule  & & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{Mini-MFRC} \\
%  & $\%B_f$ & $50\%$ &    $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\

% \midrule
% % \multicolumn{2}{c|}{MTL} & 0.417\textsubscript{(0.049)} & 0.449\textsubscript{(0.027)} & 0.418\textsubscript{(0.018)} & 0.431\textsubscript{(0.014)} & 0.763\textsubscript{(0.016)} & 0.773\textsubscript{(0.011)} & 0.772\textsubscript{(0.015)} & 0.776\textsubscript{(0.004)} \\
% % \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{bal}$} & $k=16$ & 0.442\textsubscript{(0.003)} & 0.457\textsubscript{(0.016)} & 0.458\textsubscript{(0.044)} & \cellcolor{lightgray} & 0.785\textsubscript{(0.006)} & 0.781\textsubscript{(0.004)} & 0.778\textsubscript{(0.01)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.454\textsubscript{(0.013)} & 0.469\textsubscript{(0.004)} & 0.461\textsubscript{(0.026)} & \cellcolor{lightgray} & 0.787\textsubscript{(0.006)} & 0.782\textsubscript{(0.003)} & 0.779\textsubscript{(0.012)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.462\textsubscript{(0.01)} & 0.47\textsubscript{(0.018)} & 0.467\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.788\textsubscript{(0.005)} & 0.784\textsubscript{(0.001)} & 0.782\textsubscript{(0.011)} & \cellcolor{lightgray} \\
%  & $k=128$ & \textbf{0.498\textsubscript{(0.009)}} & \textbf{0.517\textsubscript{(0.025)}} & \textbf{0.524\textsubscript{(0.021)}} & \cellcolor{lightgray} & 0.79\textsubscript{(0.005)} & 0.785\textsubscript{(0.001)} & 0.785\textsubscript{(0.01)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{dis}$} & $k=16$ & 0.399\textsubscript{(0.013)} & 0.412\textsubscript{(0.006)} & 0.457\textsubscript{(0.036)} & \cellcolor{lightgray} & 0.793\textsubscript{(0.01)} & 0.795\textsubscript{(0.004)} & 0.785\textsubscript{(0.01)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.402\textsubscript{(0.008)} & 0.413\textsubscript{(0.02)} & 0.455\textsubscript{(0.03)} & \cellcolor{lightgray} & 0.796\textsubscript{(0.01)} & 0.797\textsubscript{(0.004)} & 0.787\textsubscript{(0.011)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.429\textsubscript{(0.018)} & 0.458\textsubscript{(0.018)} & 0.518\textsubscript{(0.017)} & \cellcolor{lightgray} & 0.797\textsubscript{(0.011)} & 0.799\textsubscript{(0.005)} & 0.788\textsubscript{(0.012)} & \cellcolor{lightgray} \\
%  & $k=128$ & 0.456\textsubscript{(0.011)} & 0.476\textsubscript{(0.026)} & 0.511\textsubscript{(0.023)} & \cellcolor{lightgray} & 0.798\textsubscript{(0.009)} & 0.799\textsubscript{(0.003)} & 0.786\textsubscript{(0.012)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{mv}$} & $k=16$ & 0.409\textsubscript{(0.018)} & 0.416\textsubscript{(0.026)} & 0.442\textsubscript{(0.055)} & \cellcolor{lightgray} & 0.799\textsubscript{(0.003)} & 0.794\textsubscript{(0.004)} & 0.786\textsubscript{(0.015)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.404\textsubscript{(0.029)} & 0.426\textsubscript{(0.029)} & 0.461\textsubscript{(0.024)} & \cellcolor{lightgray} & 0.801\textsubscript{(0.003)} & 0.795\textsubscript{(0.003)} & 0.787\textsubscript{(0.017)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.409\textsubscript{(0.017)} & 0.41\textsubscript{(0.05)} & 0.467\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.802\textsubscript{(0.004)} & 0.797\textsubscript{(0.002)} & 0.79\textsubscript{(0.018)} & \cellcolor{lightgray} \\
%  & $k=128$ & 0.425\textsubscript{(0.028)} & 0.428\textsubscript{(0.035)} & 0.46\textsubscript{(0.025)} & \cellcolor{lightgray} & 0.805\textsubscript{(0.004)} & 0.798\textsubscript{(0.003)} & 0.79\textsubscript{(0.019)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \multirow[c]{4}{*}{$\mathcal{S}_{rand}$} & $k=16$ & 0.4\textsubscript{(0.017)} & 0.414\textsubscript{(0.045)} & 0.44\textsubscript{(0.037)} & \cellcolor{lightgray} & 0.815\textsubscript{(0.026)} & 0.814\textsubscript{(0.033)} & 0.805\textsubscript{(0.033)} & \cellcolor{lightgray} \\
%  & $k=32$ & 0.412\textsubscript{(0.006)} & 0.436\textsubscript{(0.026)} & 0.422\textsubscript{(0.027)} & \cellcolor{lightgray} & 0.816\textsubscript{(0.028)} & 0.815\textsubscript{(0.035)} & 0.807\textsubscript{(0.031)} & \cellcolor{lightgray} \\
%  & $k=64$ & 0.423\textsubscript{(0.02)} & 0.447\textsubscript{(0.016)} & 0.447\textsubscript{(0.019)} & \cellcolor{lightgray} & 0.818\textsubscript{(0.027)} & 0.815\textsubscript{(0.033)} & 0.809\textsubscript{(0.033)} & \cellcolor{lightgray} \\
%  & $k=128$ & 0.433\textsubscript{(0.023)} & 0.466\textsubscript{(0.006)} & 0.443\textsubscript{(0.027)} & \cellcolor{lightgray} & 0.819\textsubscript{(0.026)} & 0.816\textsubscript{(0.032)} & 0.81\textsubscript{(0.031)} & \cellcolor{lightgray} \\
% \cline{1-10}
% \bottomrule
% \end{tabular}
% \caption{Few-shot F1 results ($F_1^{fs}$) on BREXIT  and Mini-MFRC dataset for different percentages of the full budget ($\%B_f$s). Mean and standard deviation across three repeated runs.}
% \label{tab:fs_sampling}
% \end{table*}

\def\mystrut{\rule{0pt}{2\normalbaselineskip}}
\begin{table*}[ht]\small
\begin{tabular}{cl|cccc|cccc}
\toprule 
 \multicolumn{2}{c|}{\multirow{2}{*}{$metric = F_1^{fs} \uparrow$}} & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{\mf} \\
  \multicolumn{2}{c|}{} & $50\%$ & $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\
  \toprule
 \multicolumn{2}{c|}{\scriptsize{\wideunderline[7em]{$X\% \times \lvert D_{a_i} \rvert$ }}}
 % \rvert$ = \sfrac{\lvert \mathcal{A}_{mtl} \rvert}{\lvert \mathcal{A} \rvert}$}
  & \scriptsize{$50\%  \lvert D_{a_i} \rvert$} & \scriptsize{$66\%  \lvert D_{a_i} \rvert$} & \scriptsize{$83\%  \lvert D_{a_i} \rvert$} & \scriptsize{$\lvert D_{a_i} \rvert$} & \scriptsize{$25\% \lvert D_{a_i} \rvert$} & \scriptsize{$50\%  \lvert D_{a_i} \rvert$} & \scriptsize{$ 75\% \lvert D_{a_i} \rvert$} & \scriptsize{$\lvert D_{a_i} \rvert$} \\ [0.1cm]

\multicolumn{2}{c|}{MTL} & 0.417\textsubscript{(0.049)} & 0.449\textsubscript{(0.027)} & 0.418\textsubscript{(0.018)} & 0.431\textsubscript{(0.014)} & 0.763\textsubscript{(0.016)} & 0.773\textsubscript{(0.011)} & 0.772\textsubscript{(0.015)} & 0.776\textsubscript{(0.004)} \\ [0.1cm]
\toprule
 \multicolumn{2}{c|}{\scriptsize{\wideunderline[7em]{$X\% \times \lvert \mathcal{A} \rvert$ }}} 
    & \scriptsize{$50\% \lvert \mathcal{A} \rvert$} & \scriptsize{$66\% \lvert \mathcal{A} \rvert$} & \scriptsize{$83\% \lvert \mathcal{A} \rvert$} & \cellcolor{lightgray} 
    & \scriptsize{$ 25\% \lvert \mathcal{A}  \rvert$} & \scriptsize{$ 50\% \lvert \mathcal{A}  \rvert$} & \scriptsize{$ 75\% \lvert \mathcal{A}  \rvert$} & \cellcolor{lightgray}  \\ [0.1cm]
 
 % & \wideunderline[4em]{$\sfrac{3}{6}$} & \wideunderline[4em]{$\sfrac{4}{6}$} & \wideunderline[4em]{$\sfrac{5}{6}$} &  & \wideunderline[4em]{$\sfrac{6}{24}$} & \wideunderline[4em]{$\sfrac{12}{24}$} & \wideunderline[4em]{$\sfrac{18}{24}$} &  \\ [0.2cm]

\multirow[c]{4}{*}{$k=16$} & $\mathcal{S}_{bal}$ & 0.442\textsubscript{(0.003)} & 0.457\textsubscript{(0.016)} & 0.458\textsubscript{(0.044)} & \cellcolor{lightgray} & 0.785\textsubscript{(0.006)} & 0.781\textsubscript{(0.004)} & 0.778\textsubscript{(0.01)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.399\textsubscript{(0.013)} & 0.412\textsubscript{(0.006)} & 0.457\textsubscript{(0.036)} & \cellcolor{lightgray} & 0.793\textsubscript{(0.01)} & 0.795\textsubscript{(0.004)} & 0.785\textsubscript{(0.01)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.409\textsubscript{(0.018)} & 0.416\textsubscript{(0.026)} & 0.442\textsubscript{(0.055)} & \cellcolor{lightgray} & 0.799\textsubscript{(0.003)} & 0.794\textsubscript{(0.004)} & 0.786\textsubscript{(0.015)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.4\textsubscript{(0.017)} & 0.414\textsubscript{(0.045)} & 0.44\textsubscript{(0.037)} & \cellcolor{lightgray} & 0.815\textsubscript{(0.026)} & 0.814\textsubscript{(0.033)} & 0.805\textsubscript{(0.033)} & \cellcolor{lightgray} \\
\cline{1-10}
\multirow[c]{4}{*}{$k=32$} & $\mathcal{S}_{bal}$ & 0.454\textsubscript{(0.013)} & 0.469\textsubscript{(0.004)} & 0.461\textsubscript{(0.026)} & \cellcolor{lightgray} & 0.787\textsubscript{(0.006)} & 0.782\textsubscript{(0.003)} & 0.779\textsubscript{(0.012)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.402\textsubscript{(0.008)} & 0.413\textsubscript{(0.02)} & 0.455\textsubscript{(0.03)} & \cellcolor{lightgray} & 0.796\textsubscript{(0.01)} & 0.797\textsubscript{(0.004)} & 0.787\textsubscript{(0.011)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.404\textsubscript{(0.029)} & 0.426\textsubscript{(0.029)} & 0.461\textsubscript{(0.024)} & \cellcolor{lightgray} & 0.801\textsubscript{(0.003)} & 0.795\textsubscript{(0.003)} & 0.787\textsubscript{(0.017)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.412\textsubscript{(0.006)} & 0.436\textsubscript{(0.026)} & 0.422\textsubscript{(0.027)} & \cellcolor{lightgray} & 0.816\textsubscript{(0.028)} & 0.815\textsubscript{(0.035)} & 0.807\textsubscript{(0.031)} & \cellcolor{lightgray} \\
\cline{1-10}
\multirow[c]{4}{*}{$k=64$} & $\mathcal{S}_{bal}$ & 0.462\textsubscript{(0.01)} & 0.47\textsubscript{(0.018)} & 0.467\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.788\textsubscript{(0.005)} & 0.784\textsubscript{(0.001)} & 0.782\textsubscript{(0.011)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.429\textsubscript{(0.018)} & 0.458\textsubscript{(0.018)} & 0.518\textsubscript{(0.017)} & \cellcolor{lightgray} & 0.797\textsubscript{(0.011)} & 0.799\textsubscript{(0.005)} & 0.788\textsubscript{(0.012)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.409\textsubscript{(0.017)} & 0.41\textsubscript{(0.05)} & 0.467\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.802\textsubscript{(0.004)} & 0.797\textsubscript{(0.002)} & 0.79\textsubscript{(0.018)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.423\textsubscript{(0.02)} & 0.447\textsubscript{(0.016)} & 0.447\textsubscript{(0.019)} & \cellcolor{lightgray} & 0.818\textsubscript{(0.027)} & 0.815\textsubscript{(0.033)} & 0.809\textsubscript{(0.033)} & \cellcolor{lightgray} \\
\cline{1-10}
\multirow[c]{4}{*}{$k=128$} & $\mathcal{S}_{bal}$ & \textbf{0.498}\textsubscript{(0.009)} & \textbf{0.517}\textsubscript{(0.025)} & \textbf{0.524}\textsubscript{(0.021)} & \cellcolor{lightgray} & 0.79\textsubscript{(0.005)} & 0.785\textsubscript{(0.001)} & 0.785\textsubscript{(0.01)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.456\textsubscript{(0.011)} & 0.476\textsubscript{(0.026)} & 0.511\textsubscript{(0.023)} & \cellcolor{lightgray} & 0.798\textsubscript{(0.009)} & 0.799\textsubscript{(0.003)} & 0.786\textsubscript{(0.012)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.425\textsubscript{(0.028)} & 0.428\textsubscript{(0.035)} & 0.46\textsubscript{(0.025)} & \cellcolor{lightgray} & 0.805\textsubscript{(0.004)} & 0.798\textsubscript{(0.003)} & 0.79\textsubscript{(0.019)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.433\textsubscript{(0.023)} & 0.466\textsubscript{(0.006)} & 0.443\textsubscript{(0.027)} & \cellcolor{lightgray} & \textbf{0.819}\textsubscript{(0.026)} & \textbf{0.816}\textsubscript{(0.032)} & \textbf{0.81}\textsubscript{(0.031)} & \cellcolor{lightgray} \\
\cline{1-10}
\bottomrule
\end{tabular}
\caption{Few-shot $F_1$ results ($F_1^{fs}$) on BREXIT  and \mf datasets across varying percentages of the full budget ($\%B$). Mean and standard deviation calculated over three repeated runs.}
\label{tab:fs_sampling}
\vspace{-3mm}
\end{table*}



==> tables/mtl.tex <==
\begin{table*}[h!]\small
\begin{tabular}{l|llll|lllll}
\toprule  & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{mfrc} \\
$\%B_f$ & $50\%$ & $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\

\midrule
MTL & 0.417\textsubscript{(0.049)} & 0.449\textsubscript{(0.027)} & 0.418\textsubscript{(0.018)} & 0.431\textsubscript{(0.014)} & 0.763\textsubscript{(0.016)} & 0.773\textsubscript{(0.011)} & 0.772\textsubscript{(0.015)} & 0.776\textsubscript{(0.004)} \\
$F_1^{mtl}$ & 0.444\textsubscript{(0.008)} & 0.453\textsubscript{(0.015)} & 0.457\textsubscript{(0.015)} & \cellcolor{lightgray} & 0.76\textsubscript{(0.007)} & 0.778\textsubscript{(0.004)} & 0.781\textsubscript{(0.003)} & \cellcolor{lightgray} \\
\bottomrule
\end{tabular}
\caption{$F_1^{mtl}$ compared to baseline. Aggregated F1 results on BREXIT  and MFRC dataset for different $\%B_f$s of annotation, mean and std over 3  runs}
\label{tab:main_res}
\end{table*}



==> tables/mtl_fs.tex <==
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}

\begin{table*}[ht]\small
\centering
\begin{tabular}{ll|cccc|cccc}
\toprule  \multicolumn{2}{c|}{\multirow{2}{*}{$metric = F_1^{overall} \uparrow$}} & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{\mf} \\
\multicolumn{2}{c|}{} & $50\%$ & $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\
\toprule
 \multicolumn{2}{c|}{\scriptsize{\wideunderline[7em]{$X\% \times \lvert D_{a_i} \rvert$ }}}
 % \rvert$ = \sfrac{\lvert \mathcal{A}_{mtl} \rvert}{\lvert \mathcal{A} \rvert}$}
  & \scriptsize{$50\%  \lvert D_{a_i} \rvert$} & \scriptsize{$66\%  \lvert D_{a_i} \rvert$} & \scriptsize{$83\%  \lvert D_{a_i} \rvert$} & \scriptsize{$\lvert D_{a_i} \rvert$} & \scriptsize{$25\% \lvert D_{a_i} \rvert$} & \scriptsize{$50\%  \lvert D_{a_i} \rvert$} & \scriptsize{$ 75\% \lvert D_{a_i} \rvert$} & \scriptsize{$\lvert D_{a_i} \rvert$} \\ [0.1cm]

\multicolumn{2}{c|}{MTL} & 0.417\textsubscript{(0.049)} & 0.449\textsubscript{(0.027)} & 0.418\textsubscript{(0.018)} & 0.431\textsubscript{(0.014)} & 0.763\textsubscript{(0.016)} & 0.773\textsubscript{(0.011)} & 0.772\textsubscript{(0.015)} & 0.776\textsubscript{(0.004)} \\ [0.1cm]
\toprule

 \multicolumn{2}{c|}{\scriptsize{\wideunderline[7em]{$X\% \times \lvert \mathcal{A} \rvert$ }}} 
    & \scriptsize{$50\% \lvert \mathcal{A} \rvert$} & \scriptsize{$66\% \lvert \mathcal{A} \rvert$} & \scriptsize{$83\% \lvert \mathcal{A} \rvert$} & \cellcolor{lightgray} 
    & \scriptsize{$ 25\% \lvert \mathcal{A}  \rvert$} & \scriptsize{$ 50\% \lvert \mathcal{A}  \rvert$} & \scriptsize{$ 75\% \lvert \mathcal{A}  \rvert$} & \cellcolor{lightgray}  \\ [0.1cm]

Ours & $k=16$ & 0.422\textsubscript{(0.012)} & 0.44\textsubscript{(0.025)} & 0.455\textsubscript{(0.007)} & \cellcolor{lightgray} & 0.795\textsubscript{(0.009)} & 0.79\textsubscript{(0.006)} & 0.785\textsubscript{(0.005)} & \cellcolor{lightgray} \\
Ours & $k=32$ &  0.428\textsubscript{(0.006)} & 0.447\textsubscript{(0.019)} & 0.452\textsubscript{(0.016)}  & \cellcolor{lightgray} & 0.795\textsubscript{(0.01)} & 0.791\textsubscript{(0.006)} & 0.785\textsubscript{(0.004)}  & \cellcolor{lightgray} \\

Ours & $k=64$ & 0.433\textsubscript{(0.012)} & 0.451\textsubscript{(0.015)} & \textbf{0.456}\textsubscript{(0.013)}  & \cellcolor{lightgray} & 0.797\textsubscript{(0.009)} & 0.791\textsubscript{(0.006)} & 0.785\textsubscript{(0.004)}  & \cellcolor{lightgray} \\
Ours & $k=128$ & \textbf{0.439}\textsubscript{(0.015)} & \textbf{0.457}\textsubscript{(0.012)} & 0.455\textsubscript{(0.011)}  & \cellcolor{lightgray} & \textbf{0.798}\textsubscript{(0.008)} & \textbf{0.791}\textsubscript{(0.005)} & \textbf{0.786}\textsubscript{(0.004)}  & \cellcolor{lightgray} \\
\bottomrule
\end{tabular}
\caption{Mean and standard deviation of $F_1$ scores on Brexit and \mf dataset across three runs, with varying annotation budgets ($\%B$). The budget allocation differs in the baseline and our framework; For example, $50\% \lvert D_{a_i} \rvert$ indicates selecting 50\% of each annotator's data, while $50\% \lvert \mathcal{A} \rvert$  denotes selecting $50\%$ of annotators and using all their data (i.e., 3 out of 6 annotators for Brexit, and 12 out of 24 annotators for MFSC).}

\label{tab:overall-f1}
\end{table*}



% \begin{tabular}{llllllll}
% \multirow[t]{4}{*}{strategy_random} & 128 & 0.439_{(0.015)} & 0.457_{(0.012)} & 0.455_{(0.011)} & 0.798_{(0.008)} & 0.791_{(0.005)} & 0.786_{(0.004)} \\
%  & 16 & 0.422_{(0.012)} & 0.44_{(0.025)} & 0.455_{(0.007)} & 0.795_{(0.009)} & 0.79_{(0.006)} & 0.785_{(0.005)} \\
%  & 32 & 0.428_{(0.006)} & 0.447_{(0.019)} & 0.452_{(0.016)} & 0.795_{(0.01)} & 0.791_{(0.006)} & 0.785_{(0.004)} \\
%  & 64 & 0.433_{(0.012)} & 0.451_{(0.015)} & 0.456_{(0.013)} & 0.797_{(0.009)} & 0.791_{(0.006)} & 0.785_{(0.004)} \\
% \cline{1-8}
% \bottomrule
% \end{tabular}




% \begin{table*}[h!]\small
% \centering
% \label{tab:overall-f1}
% \begin{tabular}{ll|llll|llll}
% \toprule & & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{mfrc} \\
% \hdashline
% $\%B_f$ & Shots & $50\%$ & $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\
% \midrule
% MTL & \multicolumn{1}{c|}{-} & 0.417\textsubscript{(0.049)} & 0.449\textsubscript{(0.027)} & 0.418\textsubscript{(0.018)} & 0.431\textsubscript{(0.014)} & 0.763\textsubscript{(0.016)} & 0.773\textsubscript{(0.011)} & 0.772\textsubscript{(0.015)} & 0.776\textsubscript{(0.004)} \\ \hline
% Ours & $k=16$ & 0.422\textsubscript{(0.012)} & 0.44\textsubscript{(0.025)} & 0.454\textsubscript{(0.007)} & \cellcolor{lightgray} & 0.801\textsubscript{(0.019)} & 0.796\textsubscript{(0.015)} & 0.787\textsubscript{(0.008)} & \cellcolor{lightgray} \\
% Ours & $k=32$ & 0.428\textsubscript{(0.006)} & 0.447\textsubscript{(0.019)} & 0.451\textsubscript{(0.016)} & \cellcolor{lightgray} & 0.802\textsubscript{(0.02)} & 0.797\textsubscript{(0.016)} & 0.788\textsubscript{(0.007)} & \cellcolor{lightgray} \\
% Ours & $k=64$ & 0.433\textsubscript{(0.012)} & 0.451\textsubscript{(0.015)} & 0.456\textsubscript{(0.013)} & \cellcolor{lightgray} & 0.803\textsubscript{(0.02)} & 0.797\textsubscript{(0.015)} & 0.788\textsubscript{(0.008)} & \cellcolor{lightgray} \\
% Ours & $k=128$ & 0.439\textsubscript{(0.015)} & 0.458\textsubscript{(0.012)} & 0.455\textsubscript{(0.011)} & \cellcolor{lightgray} & 0.804\textsubscript{(0.018)} & 0.797\textsubscript{(0.015)} & 0.789\textsubscript{(0.008)} & \cellcolor{lightgray} \\
% \bottomrule
% \end{tabular}
% \caption{Overall F1 results on Brexit  and MFRC dataset for different budgets ($\%B_f$) of annotation, mean and standard deviation over three runs}
% \label{tab:overall-f1}
% \end{table*}

==> tables/roberta-large_fs.tex <==
\begin{table*}[h]\small


\begin{tabular}{cl|cccc|cccc}
\toprule 
 \multicolumn{2}{c|}{\multirow{2}{*}{$metric = F_1^{fs} \uparrow$}} & \multicolumn{4}{c|}{Brexit} & \multicolumn{4}{c}{\mf} \\
  \multicolumn{2}{c|}{} & $50\%$ & $66\%$ & $83\%$ & $100\%$ & $25\%$ & $50\%$ & $75\%$ & $100\%$ \\
\toprule
 \multicolumn{2}{c|}{\scriptsize{\wideunderline[7em]{$X\% \times \lvert D_{a_i} \rvert$ }}}
 % \rvert$ = \sfrac{\lvert \mathcal{A}_{mtl} \rvert}{\lvert \mathcal{A} \rvert}$}
  & \scriptsize{$50\%  \lvert D_{a_i} \rvert$} & \scriptsize{$66\%  \lvert D_{a_i} \rvert$} & \scriptsize{$83\%  \lvert D_{a_i} \rvert$} & \scriptsize{$\lvert D_{a_i} \rvert$} & \scriptsize{$25\% \lvert D_{a_i} \rvert$} & \scriptsize{$50\%  \lvert D_{a_i} \rvert$} & \scriptsize{$ 75\% \lvert D_{a_i} \rvert$} & \scriptsize{$\lvert D_{a_i} \rvert$} \\ [0.1cm]

\multicolumn{2}{c|}{MTL} & 0.366\textsubscript{(0.123)} & 0.476\textsubscript{(0.026)} & 0.497\textsubscript{(0.012)} & 0.475\textsubscript{(0.012)} & 0.773\textsubscript{(0.002)} & 0.768\textsubscript{(0.007)} & 0.772\textsubscript{(0.004)} & 0.771\textsubscript{(0.004)} \\

\toprule

\multicolumn{2}{c|}{\scriptsize{\wideunderline[7em]{$X\% \times \lvert \mathcal{A} \rvert$ }}} 
    & \scriptsize{$50\% \lvert \mathcal{A} \rvert$} & \scriptsize{$66\% \lvert \mathcal{A} \rvert$} & \scriptsize{$83\% \lvert \mathcal{A} \rvert$} & \cellcolor{lightgray} 
    & \scriptsize{$ 25\% \lvert \mathcal{A}  \rvert$} & \scriptsize{$ 50\% \lvert \mathcal{A}  \rvert$} & \scriptsize{$ 75\% \lvert \mathcal{A}  \rvert$} & \cellcolor{lightgray}  \\ [0.1cm]

\multirow[c]{4}{*}{16} & $\mathcal{S}_{bal}$ & 0.471\textsubscript{(0.004)} & 0.482\textsubscript{(0.02)} & 0.48\textsubscript{(0.012)} & \cellcolor{lightgray} & 0.782\textsubscript{(0.004)} & 0.783\textsubscript{(0.005)} & 0.758\textsubscript{(0.005)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.461\textsubscript{(0.015)} & 0.467\textsubscript{(0.004)} & 0.496\textsubscript{(0.047)} & \cellcolor{lightgray} & 0.794\textsubscript{(0.001)} & 0.8\textsubscript{(0.002)} & 0.77\textsubscript{(0.001)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.404\textsubscript{(0.105)} & 0.463\textsubscript{(0.001)} & 0.498\textsubscript{(0.122)} & \cellcolor{lightgray} & 0.793\textsubscript{(0.002)} & 0.799\textsubscript{(0.003)} & 0.769\textsubscript{(0.003)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.466\textsubscript{(0.033)} & 0.478\textsubscript{(0.01)} & 0.49\textsubscript{(0.069)} & \cellcolor{lightgray} & 0.795\textsubscript{(0.0)} & 0.797\textsubscript{(0.001)} & 0.771\textsubscript{(0.004)} & \cellcolor{lightgray} \\
\cline{1-10}
\multirow[c]{4}{*}{32} & $\mathcal{S}_{bal}$ & 0.484\textsubscript{(0.011)} & 0.491\textsubscript{(0.011)} & 0.492\textsubscript{(0.013)} & \cellcolor{lightgray} & 0.78\textsubscript{(0.003)} & 0.783\textsubscript{(0.003)} & 0.759\textsubscript{(0.001)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.462\textsubscript{(0.009)} & 0.485\textsubscript{(0.027)} & 0.476\textsubscript{(0.042)} & \cellcolor{lightgray} & 0.796\textsubscript{(0.002)} & 0.8\textsubscript{(0.001)} & 0.773\textsubscript{(0.001)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.434\textsubscript{(0.094)} & 0.464\textsubscript{(0.008)} & 0.514\textsubscript{(0.016)} & \cellcolor{lightgray} & 0.796\textsubscript{(0.002)} & 0.799\textsubscript{(0.003)} & 0.771\textsubscript{(0.001)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.482\textsubscript{(0.004)} & 0.474\textsubscript{(0.009)} & 0.488\textsubscript{(0.039)} & \cellcolor{lightgray} & 0.795\textsubscript{(0.001)} & 0.799\textsubscript{(0.001)} & 0.77\textsubscript{(0.006)} & \cellcolor{lightgray} \\
\cline{1-10}
\multirow[c]{4}{*}{64} & $\mathcal{S}_{bal}$ & 0.497\textsubscript{(0.014)} & 0.495\textsubscript{(0.003)} & 0.495\textsubscript{(0.004)} & \cellcolor{lightgray} & 0.778\textsubscript{(0.006)} & 0.783\textsubscript{(0.003)} & 0.761\textsubscript{(0.004)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.514\textsubscript{(0.002)} & 0.491\textsubscript{(0.022)} & \textbf{0.569}\textsubscript{(0.018)} & \cellcolor{lightgray} & 0.798\textsubscript{(0.001)} & 0.802\textsubscript{(0.001)} & 0.776\textsubscript{(0.001)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.447\textsubscript{(0.082)} & 0.48\textsubscript{(0.006)} & 0.509\textsubscript{(0.008)} & \cellcolor{lightgray} & 0.798\textsubscript{(0.001)} & 0.8\textsubscript{(0.002)} & 0.774\textsubscript{(0.002)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.492\textsubscript{(0.02)} & 0.492\textsubscript{(0.021)} & 0.493\textsubscript{(0.037)} & \cellcolor{lightgray} & 0.798\textsubscript{(0.002)} & 0.799\textsubscript{(0.003)} & 0.775\textsubscript{(0.004)} & \cellcolor{lightgray} \\
\cline{1-10}
\multirow[c]{4}{*}{128} & $\mathcal{S}_{bal}$ & \textbf{0.537}\textsubscript{(0.009)} & \textbf{0.531}\textsubscript{(0.018)} & 0.534\textsubscript{(0.026)} & \cellcolor{lightgray} & 0.784\textsubscript{(0.006)} & 0.786\textsubscript{(0.005)} & 0.762\textsubscript{(0.004)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{dis}$ & 0.524\textsubscript{(0.003)} & 0.512\textsubscript{(0.009)} & 0.559\textsubscript{(0.031)} & \cellcolor{lightgray} & \textbf{0.8}\textsubscript{(0.001)} & \textbf{0.806}\textsubscript{(0.002)} & \textbf{0.778}\textsubscript{(0.001)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{mv}$ & 0.438\textsubscript{(0.109)} & 0.5\textsubscript{(0.001)} & 0.523\textsubscript{(0.007)} & \cellcolor{lightgray} & 0.799\textsubscript{(0.002)} & 0.803\textsubscript{(0.001)} & 0.777\textsubscript{(0.003)} & \cellcolor{lightgray} \\
 & $\mathcal{S}_{rand}$ & 0.503\textsubscript{(0.011)} & 0.509\textsubscript{(0.026)} & 0.541\textsubscript{(0.012)} & \cellcolor{lightgray} & 0.8\textsubscript{(0.002)} & 0.802\textsubscript{(0.001)} & 0.78\textsubscript{(0.003)} & \cellcolor{lightgray} \\
\cline{1-10}
\bottomrule
\end{tabular}
\caption{\textbf{Roberta-large} few shot  Aggregated F1 results on BREXIT  and MFRC dataset for different $\%B_f$s of annotation, mean and std over 3  runs}
\label{tab:roberta-large_fs}
\end{table*}


